Intermediate-Mass Black Holes in Star Clusters and Dwarf Galaxies

Black holes (BHs) with masses between 100 to 100,000 times the mass of the Sun ($\rm{M}_{\odot}$) are classified as intermediate-mass black holes (IMBHs), potentially representing a crucial link between stellar-mass and supermassive BHs. Stellar-mass BHs are endpoints of the evolution of stars initially more massive than roughly 20 $\rm{M}_{\odot}$ and generally weigh about 10 to 100 $\rm{M}_{\odot}$. Supermassive BHs are found in the centre of many galaxies and weigh between $10^{6}$ to $10^{10} \ \rm{M}_{\odot}$. The origin of supermassive BHs remains an unresolved problem in astrophysics, with many viable pathways suggesting that they undergo an intermediate-mass phase. Whether IMBHs really stand as an independent category of BHs or rather they represent the heaviest stellar mass and the lightest supermassive BHs is still unclear, mostly owing to the lack of an observational smoking gun. The first part of this chapter discusses proposed formation channels of IMBHs and focuses on their formation and growth in dense stellar environments like globular and nuclear star clusters. It also highlights how the growth of IMBHs through mergers with other BHs is important from the point of view of gravitational waves and seeding of supermassive BHs in our Universe. The second part of the chapter focuses on the multi-wavelength observational constraints on IMBHs in dense star clusters and dwarf galactic nuclei. It also examines the potential insights that future gravitational wave detectors could offer in unraveling the mystery surrounding IMBHs.

==> Acronyms.tex <==
%BLACK HOLES
\acrodef{GW}{Gravitational wave}
\acrodefplural{GW}[GWs]{Gravitational waves}

\acrodef{BH}{Black hole}
\acrodefplural{BH}[BHs]{Black holes}

\acrodef{BBH}{binary black hole}
\acrodefplural{BBH}[BBHs]{binary black holes}

\acrodef{IMBH}{intermediate-mass black hole}
\acrodefplural{IMBH}[IMBHs]{intermediate-mass black holes}

\acrodef{SMBH}{supermassive black hole}
\acrodefplural{SMBH}[SMBHs]{supermassive black holes}

\acrodef{PBH}{primordial black hole}
\acrodefplural{PBH}[PBHs]{primordial black holes}


% CLUSTERS AND GALACTIC ENVIRONS
\acrodef{GC}{globular cluster}
\acrodefplural{GC}[GCs]{globular clusters}

\acrodef{NC}{nuclear cluster}
\acrodefplural{NC}[NCs]{nuclear clusters}

\acrodef{OC}{open cluster}
\acrodefplural{OC}[OCs]{open clusters}

\acrodef{YMC}{young massive cluster}
\acrodefplural{YMC}[YMCs]{young massive clusters}


% STARS AND COMPACT OBJECTS
\acrodef{MLT}{mixing-length theory}
\acrodef{HR}{Hertzsprung-Russell}
\acrodef{MS}{main sequence}
\acrodef{ZAMS}{zero-age MS}
\acrodef{CHeB}{core helium burning}
\acrodef{RGB}{red giant branch}
\acrodef{RG}{red giant}
\acrodef{RSG}{red super-giant}
\acrodef{HB}{horizontal branch}
\acrodef{AGB}{asymptotic giant branch}
\acrodef{TP-AGB}{thermally-pulsating asymptotic giant branch}
\acrodef{LBV}{luminous blue variable}
\acrodef{WR}{Wolf-Rayet}

\acrodef{WD}{white dwarf}
\acrodefplural{WDs}{white dwarfs}
\acrodef{NS}{neutron star}
\acrodefplural{NSs}{neutron stars}
\acrodef{CO}{compact object}
\acrodefplural{COs}{compact objects}

\acrodef{CC}{core collapse}
\acrodef{ECSN}{electron-capture supernova}
\acrodef{PI}{pair instability}
\acrodef{PISN}{pair instability supernova}
\acrodef{PPISN}{pulsational pair instability supernova}

\acrodef{RLOF}{Roche lobe overflow}

% CODES (USE \TEXTTT)
\acrodef{compas}{\texttt{COMPAS}}
\acrodef{mobse}{\texttt{MOBSE}}
%



%BLACK HOLES
%\acrodef{BH}{black hole}
%\acrodefplural{BH}[BHs]{black holes}

\acrodef{cBH}{Black hole}
\acrodefplural{cBH}[BHs]{Black holes}

\acrodef{sBH}{stellar-mass black hole}
\acrodefplural{sBH}[sBHs]{Stellar-mass black holes}

\acrodef{IMBH}{intermediate-mass black hole}
\acrodefplural{IMBH}[IMBHs]{intermediate-mass black holes}

\acrodef{SMBH}{supermassive black hole}
\acrodefplural{SMBH}[SMBHs]{Supermassive black holes}

\acrodef{IMRI}{intermediate-mass ratio inspiral}
\acrodefplural{IMRI}[IMRIs]{intermediate-mass ratio inspirals}

\acrodef{BBH}{binary black hole}
\acrodefplural{BBH}{binary black holes}

% CLUSTERS AND GALACTIC ENVIRONS
\acrodef{GC}{globular cluster}
\acrodefplural{GC}[GCs]{Globular clusters}

\acrodef{NSC}{nuclear star cluster}
\acrodefplural{NSC}[NSCs]{Nuclear star clusters}

\acrodef{OC}{open cluster}
\acrodefplural{OC}[OCs]{open clusters}

\acrodef{YMC}{young massive cluster}
\acrodefplural{YMC}[YMCs]{Young massive clusters}

\acrodef{AGN}[AGN]{active galactic nucleus}
\acrodefplural{AGN}[AGNs]{active galactic nuclei}



%Processes

\acrodef{IMF}{initial mass function}

% \acrodef{GW}[GW]{gravitational wave}
% \acrodefplural{GW}[GWs]{gravitational waves}
%Missions
\acrodef{LVK}[LW]{LIGO-Virgo-KAGRA collaboration}
\acrodef{LISA}{Laser Interferometer Space Antenna}

\acrodef{PTA}[PTA]{Pulsar Timing Array}
\acrodefplural{PTA}[PTAs]{Pulsar Timing Arrays}

% STARS AND COMPACT OBJECTS
\acrodef{VMS}{very massive star}
\acrodefplural{VMSs}[VMS]{very massive stars}

\acrodef{ZAMS}{zero-age main sequence}
\acrodef{MS}{main sequence}
\acrodef{WD}{white dwarf}
\acrodefplural{WDs}{white dwarfs}
\acrodef{NS}{neutron star}
\acrodefplural{NSs}{neutron stars}
\acrodef{CO}{compact object}
\acrodefplural{COs}{compact objects}

%galaxies etc

\acrodef{MW}{Milky Way}

% CODES (USE \TEXTTT)
\acrodef{SSE}{\texttt{SSE}}
\acrodef{BSE}{\texttt{BSE}}
\acrodef{MOCCA}{\texttt{MOCCA}}


==> Symbols.tex <==
%Z = metallicity
\newcommand{\Ms}{{\rm M}_\odot} 
\newcommand{\Rs}{{\rm R}_\odot}
\newcommand{\Zs}{{\rm Z}_\odot}
\newcommand{\AU}{{\rm AU}}
\newcommand{\pc}{{\rm pc}}
\newcommand{\Mzams}{{\rm M}_{\rm ZAMS}}
\newcommand{\kms}{{\rm {km\, s^{-1}}}}
\newcommand{\msun}{{\rm M_{\odot}}}
\newcommand{\Mo}{\msun}
\newcommand{\Ro}{{\rm R_{\sun }}}
\newcommand{\Lo}{{\rm L_{\sun }}}
%\newcommand{\Teff}{T_{\rm eff}}
\newcommand{\ud}{{\rm d}}
\newcommand{\s}{{\rm s}}
\def\Mc{M_{\rm c}}
\def\Rc{R_{\rm c}}
\def\r{{\tilde{r}}}
\def\vt{{\tilde{v}}}
\newcommand{\red}{\color{red}}
\newcommand{\ri}{\color{red}\it}
\newcommand{\blue}{\color{blue}}




==> Typographic_Rules.tex <==

 - Abbreviations: Their use is minimised. For instance, we write Figure instead of Fig., Table instead Tab. etc.

 - Acronyms: Their use is minimised. Note that we write out "gravitational waves" or "dark matter", except when these words would appear as sub- or superscripts.

 - Bibliography 1: We use "\interlinepenalty=10000" (directly before the bibliography) in order to avoid splitting bibliography entries.

 - Bibliography 2: We use "\setlength{\bibsep}{6pt}" in order to induce a bit more space between bibliographic entries. 

 - Boxes: Important lists and statements are boxed with a newly-defined light-grey box environment, defined as "newquote" in our header file "PBH-header-tex", which we include at the beginning at the document:

 "\usepackage[most]{tcolorbox}
 \definecolor{block-gray}{gray}{0.92}
 \newtcolorbox{newquote}{colback=block-gray, grow to right by=-5mm, grow to left by=-5mm, boxrule=1pt, boxsep=5pt, breakable}"

 - Brackets: Here, LaTeX puts by default too much space in from of some exponents, for instance at large round delimiters such as "\Bigg)^{...}". Hence, we add a negative space in the exponent, depending on kind and size of the bracket, for instance "\Bigg)^{\mspace{-6mu}...}".

 - Capitals: We write the first letter of (our/the) Earth, (the) Universe, (the) Nature, (our) Galaxy (which we also call Milky Way) etc. in capital, as opposed to "other galaxies" for instance. Also, we write the "Standard Model" of particle physical.

 - Commata: In a list within a mathematical environment, in which the elements are separated by commata, we include separators such as in "$A(r,\mspace{1.5mu}t)$" instead of "$A(r,t)$".
 
 - Dashes 1: We use single ones (-) in words like "saddle-point equations", double ones (--) for names like "Fokker--Planck", triple ones (---) for dashes in the text, which we apply between two words (say, WORD-1 & WORD-2) as WORD-1{\,---\,}WORD-2.

 - Dashes 2: Generally, for three words A, B and C, which should read (A B) C, we write A-B C, such as in "saddle-point equations", or "gravitational-wave observatories". Exceptions are the words "black hole" and "dark matter" which are singular terms and shall not be connected with a dash.

 - Definitions: We use "\coloneqq" or "\eqqcolon" to define quantities.

 - Differentials: These are written in regular (not in italic), since they are not variables, such as in "\d f(r) / \d r", where "\d" has been redefined via "\renewcommand{\d}{\ensuremath{\mathrm{d}}}".

 - Dimensions/Margins: We use the following page dimensions:

 "\textwidth=150mm
 \textheight=214mm
 \hoffset=7.525mm
 \footskip=18mm

 \headwidth=\textwidth

 \setlength{\headheight}{32pt}
 \renewcommand{\headrulewidth}{0.1mm}
 \setlength{\headsep}{8mm}"

 - Drop Caps: Each section starts with a drop cap, using the package "lettrine". We use the command options "[lines=3, slope=0em, findent=0em, nindent=0.2em, lhang=0.1, loversize=0.1]"

 - English: We use British English. (Note, in particular, there is no comma after i.e. or e.g.)

 - Equation Environment: We use "align" as often as possible.

 - Equations: The punctuation marks (; , .) at the end of an equation are generally separated by a "\," horizontal space command (being equivalent to "3mu" in mathematical mode), except if the equation environment such (as "left-right") automatically adds sufficient space, such that there is no need to add additional space.

 - Font: We use the (serif) font "TEX Gyre Pagella", using the package "tgpagella" see (https://ctan.org/pkg/tex-gyre-pagella?lang=en ), which we set in 12pt size. (from the linked website: "The TEX Gyre Pagella family of serif fonts is based on URW Palladio L. The original font, Palatino, was designed by Hermann Zapf in the 1940s for the Stempel type foundry.")

 - Footer: We let the page number appear on pages in the format "-- CURRENT PAGE / LAST PAGE", e.g., "-- 14 / 212 --", using 
 
  "\cfoot{ \fancyplain{}{-- \thepage}/{\color{red}\pageref{LastPage}} -- }"

 - Footnotes: We slightly increase the space above footnotes, setting \setlength{\footnotesep}{3.5mm}

 - Header: We put the chapter's name into the header (above the horizontal line) via

 "\fancyhf{}
 \chead[odd]{
 {\bf P}rimordial 
 {\bf B}lack 
 {\bf H}oles}"

 - LaTeX Structure of Equations: These generally have one indent for the left-hand side, then -- in a new line -- two indents for the relation sign (such as "=", "<", "or ">"), and then -- in yet a new line -- three indents for the right-hand side.

 - Lines: We slightly increase spread between two lines via "\linespread{1.15}"

 - Paragraphs 1: We try to make pages end on paragraph where possible. In particular, we avoid that a single sentence is disconnected from a paragraph. In order to achieve this, we adjust vertical spaces and/or use the page break command "\newpage".

 - Paragraphs 2: We slightly increase the space between two paragraphs, setting "\setlength{\parskip}\smallskipamount".

 - Percentage Signs: These are separated from the numerical value by "\mspace{0.5mu}".

 - Plurals: We write supernov{\ae} and formul{\ae}.

 - References: When referring to a specific figure, section etc., we write this first letter in capital, such as in "This is shown in Figure~\ref{fig:...}".

 - Section Headings 1: These are slightly enlarged as compared to the subsection headings using.
 
 "\titleformat{\section}{\centering\normalfont\fontsize{14}{17}\bfseries}{\thesection}{1em}{}"

 - Section Headings 2: These are set slightly closer (vertically) to the first paragraph (by 3mm).

 - Sections: These start on a new odd page.

 - Sub-/Superscripts 1: Variable are slated, while names/acronyms are not.

 - Sub-/Superscripts 2: In some cases, they are too close or too distant from the base character and are hence slightly moved horizontally, for instance "R\mspace{1mu}'" instead of "R'", or "G$_${\mspace{-2mu}\Nrm}" instead of "G$_${\Nrm}".

 - Subsection Headings: These are set slightly closer (vertically) to the first paragraph (by 1mm).

 - Table of Contents: We remove "subsubsections" form the table of contents via
 
 "\makeatletter
 \def\l@subsubsection#1#2{}
 \makeatother"

 - Units: These are separated from the numerical value in front of them by a horizontal space of 0.5mm, for which we redefined the "\." command.



==> header.tex <==
% ******************************************************
% ********************** BEGIN HEADER **********************
% ******************************************************

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%PACKAGES
\usepackage{physics,braket}
\usepackage{amsmath}	% AMS Math Package
\usepackage{amsthm}		% Theorem Formatting
\usepackage{amssymb}	% Math symbols such as \mathbb
\usepackage{mathrsfs,mathtools}
\usepackage{datetime}
\usepackage{graphicx}
\usepackage{color}
\usepackage{verbatim}
\usepackage{bm}
\usepackage{float}
\usepackage{xcolor}
\usepackage{acronym}
\usepackage{rotating}
\usepackage{setspace}
\usepackage{aas_macros}
\usepackage{siunitx}
\usepackage[colorlinks=true
,urlcolor=DARKBLUE
,anchorcolor=DARKBLUE
,citecolor=DARKBLUE
,filecolor=DARKBLUE
,linkcolor=DARKBLUE
,menucolor=DARKBLUE
%,pagecolor=DARKBLUE
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}
%\hypersetup{
 %   colorlinks,
  %  linkcolor={red!50!black},
   % citecolor={blue!50!black},
    %urlcolor={blue!80!black}
%}

\numberwithin{equation}{section}
\renewcommand{\figurename}{{\bf Figure}}
\renewcommand{\tablename}{{\bf Table}}
\makeatletter 
\renewcommand{\thefigure}{{\bf\@arabic\c@figure}}
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%COLOURS
%existing: black, white, blue, red, green, yellow
\definecolor{grey}{rgb}{0.4,0.4,0.4}
\definecolor{dullmagenta}{rgb}{0.4,0,0.4}
\definecolor{darkblue}{rgb}{0,0,0.4}
\definecolor{midblue}{rgb}{0,0,0.7}
\definecolor{midred}{rgb}{0.5,0,0}
\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{lightbrown}{rgb}{0.75,0.5,0.25}
\definecolor{tan}{cmyk}{0.14,0.42,0.56,0}
\definecolor{djunglegreen}{cmyk}{0.99,0,0.52,0}
\definecolor{lightgreen}{rgb}{0,1,0}
\definecolor{olivegreen}{cmyk}{0.64,0,0.95,0.40}
\definecolor{midgreen}{rgb}{0.0,0.675,0.0}
\definecolor{darkgreen}{rgb}{0,0.5,0}

\definecolor{MONZA}{HTML}{CF000F}
\definecolor{DARKBLUE}{HTML}{00008b}
\definecolor{DARKMAGENTA}{HTML}{8b008b}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%NORMS
\newcommand{\normsingle}[1]{\left|{#1}\right|}
\newcommand{\normdouble}[1]{\left\|{#1}\right\|}
%\newcommand{\normtriple}[1]{\left\interleave{#1}\right\interleave} % requires ``stmaryrd'' package
%\newcommand{\norm}[1]{\normdouble{#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%SHIFTS
\newcommand{\q}{\quad}
%\newcommand{\qq}{\qquad}
\newcommand{\qqq}{\qquad\quad}
\newcommand{\qqqq}{\qquad\qquad}
\newcommand{\vs}{\vspace}
\newcommand{\hs}{\hspace}
\renewcommand{\.}{\hspace{0.5mm}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%ARROWS
\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\la}{\ensuremath{\leftarrow}}
\newcommand{\Ra}{\ensuremath{\Rightarrow}}
\newcommand{\La}{\ensuremath{\Leftarrow}}
\newcommand{\lra}{\ensuremath{\leftrightarrow}}
\newcommand{\Lra}{\ensuremath{\Leftrightarrow}}
\newcommand{\Ral}{\ensuremath{\Longrightarrow}}
\newcommand{\Lal}{\ensuremath{\Longleftarrow}}
\newcommand{\Lral}{\ensuremath{\Longleftrightarrow}}
\newcommand{\lral}{\ensuremath{\ongleftrightarrow}}
\newcommand{\ral}{\ensuremath{\longrightarrow}}
\newcommand{\lal}{\ensuremath{\longleftarrow}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%MATHEMATICS

%%%capital \mathrm
\newcommand{\Arm}{\ensuremath{\mathrm{A}}}
\newcommand{\Brm}{\ensuremath{\mathrm{B}}}
\newcommand{\Crm}{\ensuremath{\mathrm{C}}}
\newcommand{\Drm}{\ensuremath{\mathrm{D}}}
\newcommand{\Erm}{\ensuremath{\mathrm{E}}}
\newcommand{\Frm}{\ensuremath{\mathrm{F}}}
\newcommand{\Grm}{\ensuremath{\mathrm{G}}}
\newcommand{\Hrm}{\ensuremath{\mathrm{H}}}
\newcommand{\Irm}{\ensuremath{\mathrm{I}}}
\newcommand{\Jrm}{\ensuremath{\mathrm{J}}}
\newcommand{\Krm}{\ensuremath{\mathrm{K}}}
\newcommand{\Lrm}{\ensuremath{\mathrm{L}}}
\newcommand{\Mrm}{\ensuremath{\mathrm{M}}}
\newcommand{\Nrm}{\ensuremath{\mathrm{N}}}
\newcommand{\Orm}{\ensuremath{\mathrm{O}}}
\newcommand{\Prm}{\ensuremath{\mathrm{P}}}
\newcommand{\Qrm}{\ensuremath{\mathrm{Q}}}
\newcommand{\Rrm}{\ensuremath{\mathrm{R}}}
\newcommand{\Srm}{\ensuremath{\mathrm{S}}}
\newcommand{\Trm}{\ensuremath{\mathrm{T}}}
\newcommand{\Urm}{\ensuremath{\mathrm{U}}}
\newcommand{\Vrm}{\ensuremath{\mathrm{V}}}
\newcommand{\Wrm}{\ensuremath{\mathrm{W}}}
\newcommand{\Xrm}{\ensuremath{\mathrm{X}}}
\newcommand{\Yrm}{\ensuremath{\mathrm{Y}}}
\newcommand{\Zrm}{\ensuremath{\mathrm{Z}}}
%%%small \mathrm
\newcommand{\arm}{\ensuremath{\mathrm{a}}}
\newcommand{\brm}{\ensuremath{\mathrm{b}}}
\newcommand{\crm}{\ensuremath{\mathrm{c}}}
\newcommand{\drm}{\ensuremath{\mathrm{d}}}
\newcommand{\erm}{\ensuremath{\mathrm{e}}}
\newcommand{\frm}{\ensuremath{\mathrm{f}}}
\newcommand{\grm}{\ensuremath{\mathrm{g}}}
\newcommand{\hrm}{\ensuremath{\mathrm{h}}}
\newcommand{\irm}{\ensuremath{\mathrm{i}}}
\newcommand{\jrm}{\ensuremath{\mathrm{j}}}
\newcommand{\krm}{\ensuremath{\mathrm{k}}}
\newcommand{\lrm}{\ensuremath{\mathrm{l}}}
\newcommand{\mrm}{\ensuremath{\mathrm{m}}}
\newcommand{\nrm}{\ensuremath{\mathrm{n}}}
\newcommand{\orm}{\ensuremath{\mathrm{o}}}
\newcommand{\prm}{\ensuremath{\mathrm{p}}}
\newcommand{\qrm}{\ensuremath{\mathrm{q}}}
\newcommand{\rrm}{\ensuremath{\mathrm{r}}}
\newcommand{\srm}{\ensuremath{\mathrm{s}}}
\newcommand{\trm}{\ensuremath{\mathrm{t}}}
\newcommand{\urm}{\ensuremath{\mathrm{u}}}
\newcommand{\vrm}{\ensuremath{\mathrm{v}}}
\newcommand{\wrm}{\ensuremath{\mathrm{w}}}
\newcommand{\xrm}{\ensuremath{\mathrm{x}}}
\newcommand{\yrm}{\ensuremath{\mathrm{y}}}
\newcommand{\zrm}{\ensuremath{\mathrm{z}}}

%%%capital \mathcal
\newcommand{\Acal}{\ensuremath{\mathcal{A}}}
\newcommand{\Bcal}{\ensuremath{\mathcal{B}}}
\newcommand{\Ccal}{\ensuremath{\mathcal{C}}}
\newcommand{\Dcal}{\ensuremath{\mathcal{D}}}
\newcommand{\Ecal}{\ensuremath{\mathcal{E}}}
\newcommand{\Fcal}{\ensuremath{\mathcal{F}}}
\newcommand{\Gcal}{\ensuremath{\mathcal{G}}}
\newcommand{\Hcal}{\ensuremath{\mathcal{H}}}
\newcommand{\Ical}{\ensuremath{\mathcal{I}}}
\newcommand{\Jcal}{\ensuremath{\mathcal{J}}}
\newcommand{\Kcal}{\ensuremath{\mathcal{K}}}
\newcommand{\Lcal}{\ensuremath{\mathcal{L}}}
\newcommand{\Mcal}{\ensuremath{\mathcal{M}}}
\newcommand{\Ncal}{\ensuremath{\mathcal{N}}}
\newcommand{\Ocal}{\ensuremath{\mathcal{O}}}
\newcommand{\Pcal}{\ensuremath{\mathcal{P}}}
\newcommand{\Qcal}{\ensuremath{\mathcal{Q}}}
\newcommand{\Rcal}{\ensuremath{\mathcal{R}}}
\newcommand{\Scal}{\ensuremath{\mathcal{S}}}
\newcommand{\Tcal}{\ensuremath{\mathcal{T}}}
\newcommand{\Ucal}{\ensuremath{\mathcal{U}}}
\newcommand{\Vcal}{\ensuremath{\mathcal{V}}}
\newcommand{\Wcal}{\ensuremath{\mathcal{W}}}
\newcommand{\Xcal}{\ensuremath{\mathcal{X}}}
\newcommand{\Ycal}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zcal}{\ensuremath{\mathcal{Z}}}

%%%capital \mathsf
\newcommand{\Asf}{\ensuremath{\mathsf{A}}}
\newcommand{\Bsf}{\ensuremath{\mathsf{B}}}
\newcommand{\Csf}{\ensuremath{\mathsf{C}}}
\newcommand{\Dsf}{\ensuremath{\mathsf{D}}}
\newcommand{\Esf}{\ensuremath{\mathsf{E}}}
\newcommand{\Fsf}{\ensuremath{\mathsf{F}}}
\newcommand{\Gsf}{\ensuremath{\mathsf{G}}}
\newcommand{\Hsf}{\ensuremath{\mathsf{H}}}
\newcommand{\Isf}{\ensuremath{\mathsf{I}}}
\newcommand{\Jsf}{\ensuremath{\mathsf{J}}}
\newcommand{\Ksf}{\ensuremath{\mathsf{K}}}
\newcommand{\Lsf}{\ensuremath{\mathsf{L}}}
\newcommand{\Msf}{\ensuremath{\mathsf{M}}}
\newcommand{\Nsf}{\ensuremath{\mathsf{N}}}
\newcommand{\Osf}{\ensuremath{\mathsf{O}}}
\newcommand{\Psf}{\ensuremath{\mathsf{P}}}
\newcommand{\Qsf}{\ensuremath{\mathsf{Q}}}
\newcommand{\Rsf}{\ensuremath{\mathsf{R}}}
\newcommand{\Ssf}{\ensuremath{\mathsf{S}}}
\newcommand{\Tsf}{\ensuremath{\mathsf{T}}}
\newcommand{\Usf}{\ensuremath{\mathsf{U}}}
\newcommand{\Vsf}{\ensuremath{\mathsf{V}}}
\newcommand{\Wsf}{\ensuremath{\mathsf{W}}}
\newcommand{\Xsf}{\ensuremath{\mathsf{X}}}
\newcommand{\Ysf}{\ensuremath{\mathsf{Y}}}
\newcommand{\Zsf}{\ensuremath{\mathsf{Z}}}
%%%small \mathcal
\newcommand{\asf}{\ensuremath{\mathsf{a}}}
\newcommand{\bsf}{\ensuremath{\mathsf{b}}}
\newcommand{\csf}{\ensuremath{\mathsf{c}}}
\newcommand{\dsf}{\ensuremath{\mathsf{d}}}
\newcommand{\esf}{\ensuremath{\mathsf{e}}}
\newcommand{\fsf}{\ensuremath{\mathsf{f}}}
\newcommand{\gsf}{\ensuremath{\mathsf{g}}}
\newcommand{\hsf}{\ensuremath{\mathsf{h}}}
\newcommand{\isf}{\ensuremath{\mathsf{i}}}
\newcommand{\jsf}{\ensuremath{\mathsf{j}}}
\newcommand{\ksf}{\ensuremath{\mathsf{k}}}
\newcommand{\lsf}{\ensuremath{\mathsf{l}}}
\newcommand{\msf}{\ensuremath{\mathsf{m}}}
\newcommand{\nsf}{\ensuremath{\mathsf{n}}}
\newcommand{\osf}{\ensuremath{\mathsf{o}}}
\newcommand{\psf}{\ensuremath{\mathsf{p}}}
\newcommand{\qsf}{\ensuremath{\mathsf{q}}}
\newcommand{\rsf}{\ensuremath{\mathsf{r}}}
\newcommand{\ssf}{\ensuremath{\mathsf{s}}}
\newcommand{\tsf}{\ensuremath{\mathsf{t}}}
\newcommand{\usf}{\ensuremath{\mathsf{u}}}
\newcommand{\vsf}{\ensuremath{\mathsf{v}}}
\newcommand{\wsf}{\ensuremath{\mathsf{w}}}
\newcommand{\xsf}{\ensuremath{\mathsf{x}}}
\newcommand{\ysf}{\ensuremath{\mathsf{y}}}
\newcommand{\zsf}{\ensuremath{\mathsf{z}}}

%%%capital \mathbb
\newcommand{\Abb}{\ensuremath{\mathbb{A}}}
\renewcommand{\Bbb}{\ensuremath{\mathbb{B}}}
\newcommand{\Cbb}{\ensuremath{\mathbb{C}}}
\newcommand{\Dbb}{\ensuremath{\mathbb{D}}}
\newcommand{\Ebb}{\ensuremath{\mathbb{E}}}
\newcommand{\Fbb}{\ensuremath{\mathbb{F}}}
\newcommand{\Gbb}{\ensuremath{\mathbb{G}}}
\newcommand{\Hbb}{\ensuremath{\mathbb{H}}}
\newcommand{\Ibb}{\ensuremath{\mathbb{I}}}
\newcommand{\Jbb}{\ensuremath{\mathbb{J}}}
\newcommand{\Kbb}{\ensuremath{\mathbb{K}}}
\newcommand{\Lbb}{\ensuremath{\mathbb{L}}}
\newcommand{\Mbb}{\ensuremath{\mathbb{M}}}
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}}
\newcommand{\Obb}{\ensuremath{\mathbb{O}}}
\newcommand{\Pbb}{\ensuremath{\mathbb{P}}}
\newcommand{\Qbb}{\ensuremath{\mathbb{Q}}}
\newcommand{\Rbb}{\ensuremath{\mathbb{R}}}
\newcommand{\Sbb}{\ensuremath{\mathbb{S}}}
\newcommand{\Tbb}{\ensuremath{\mathbb{T}}}
\newcommand{\Ubb}{\ensuremath{\mathbb{U}}}
\newcommand{\Vbb}{\ensuremath{\mathbb{V}}}
\newcommand{\Wbb}{\ensuremath{\mathbb{W}}}
\newcommand{\Xbb}{\ensuremath{\mathbb{X}}}
\newcommand{\Ybb}{\ensuremath{\mathbb{Y}}}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z}}}
%%%small \mathbb
\newcommand{\abb}{\ensuremath{\mathbb{a}}}
\newcommand{\bbb}{\ensuremath{\mathbb{b}}}
\newcommand{\cbb}{\ensuremath{\mathbb{c}}}
\newcommand{\dbb}{\ensuremath{\mathbb{d}}}
\newcommand{\ebb}{\ensuremath{\mathbb{e}}}
\newcommand{\fbb}{\ensuremath{\mathbb{f}}}
\newcommand{\gbb}{\ensuremath{\mathbb{g}}}
\newcommand{\hbb}{\ensuremath{\mathbb{h}}}
\newcommand{\ibb}{\ensuremath{\mathbb{i}}}
\newcommand{\jbb}{\ensuremath{\mathbb{j}}}
\newcommand{\kbb}{\ensuremath{\mathbb{k}}}
\newcommand{\lbb}{\ensuremath{\mathbb{l}}}
\newcommand{\mbb}{\ensuremath{\mathbb{m}}}
\newcommand{\nbb}{\ensuremath{\mathbb{n}}}
\newcommand{\obb}{\ensuremath{\mathbb{o}}}
\newcommand{\pbb}{\ensuremath{\mathbb{p}}}
\newcommand{\qbb}{\ensuremath{\mathbb{q}}}
\newcommand{\rbb}{\ensuremath{\mathbb{r}}}
\newcommand{\sbb}{\ensuremath{\mathbb{s}}}
\newcommand{\tbb}{\ensuremath{\mathbb{t}}}
\newcommand{\ubb}{\ensuremath{\mathbb{u}}}
\newcommand{\vbb}{\ensuremath{\mathbb{v}}}
\newcommand{\wbb}{\ensuremath{\mathbb{w}}}
\newcommand{\xbb}{\ensuremath{\mathbb{x}}}
\newcommand{\ybb}{\ensuremath{\mathbb{y}}}
\newcommand{\zbb}{\ensuremath{\mathbb{z}}}

%%%capital \mathbbm
\newcommand{\Abbm}{\ensuremath{\mathbbm{A}}}
\newcommand{\Bbbm}{\ensuremath{\mathbbm{B}}}
\newcommand{\Cbbm}{\ensuremath{\mathbbm{C}}}
\newcommand{\Dbbm}{\ensuremath{\mathbbm{D}}}
\newcommand{\Ebbm}{\ensuremath{\mathbbm{E}}}
\newcommand{\Fbbm}{\ensuremath{\mathbbm{F}}}
\newcommand{\Gbbm}{\ensuremath{\mathbbm{G}}}
\newcommand{\Hbbm}{\ensuremath{\mathbbm{H}}}
\newcommand{\Ibbm}{\ensuremath{\mathbbm{I}}}
\newcommand{\Jbbm}{\ensuremath{\mathbbm{J}}}
\newcommand{\Kbbm}{\ensuremath{\mathbbm{K}}}
\newcommand{\Lbbm}{\ensuremath{\mathbbm{L}}}
\newcommand{\Mbbm}{\ensuremath{\mathbbm{M}}}
\newcommand{\Nbbm}{\ensuremath{\mathbbm{N}}}
\newcommand{\Obbm}{\ensuremath{\mathbbm{O}}}
\newcommand{\Pbbm}{\ensuremath{\mathbbm{P}}}
\newcommand{\Qbbm}{\ensuremath{\mathbbm{Q}}}
\newcommand{\Rbbm}{\ensuremath{\mathbbm{R}}}
\newcommand{\Sbbm}{\ensuremath{\mathbbm{S}}}
\newcommand{\Tbbm}{\ensuremath{\mathbbm{T}}}
\newcommand{\Ubbm}{\ensuremath{\mathbbm{U}}}
\newcommand{\Vbbm}{\ensuremath{\mathbbm{V}}}
\newcommand{\Wbbm}{\ensuremath{\mathbbm{W}}}
\newcommand{\Xbbm}{\ensuremath{\mathbbm{X}}}
\newcommand{\Ybbm}{\ensuremath{\mathbbm{Y}}}
\newcommand{\Zbbm}{\ensuremath{\mathbbm{Z}}}
%%%small \mathbbm
\newcommand{\abbm}{\ensuremath{\mathbbm{a}}}
\newcommand{\bbbm}{\ensuremath{\mathbbm{b}}}
\newcommand{\cbbm}{\ensuremath{\mathbbm{c}}}
\newcommand{\dbbm}{\ensuremath{\mathbbm{d}}}
\newcommand{\ebbm}{\ensuremath{\mathbbm{e}}}
\newcommand{\fbbm}{\ensuremath{\mathbbm{f}}}
\newcommand{\gbbm}{\ensuremath{\mathbbm{g}}}
\newcommand{\hbbm}{\ensuremath{\mathbbm{h}}}
\newcommand{\ibbm}{\ensuremath{\mathbbm{i}}}
\newcommand{\jbbm}{\ensuremath{\mathbbm{j}}}
\newcommand{\kbbm}{\ensuremath{\mathbbm{k}}}
\newcommand{\lbbm}{\ensuremath{\mathbbm{l}}}
\newcommand{\mbbm}{\ensuremath{\mathbbm{m}}}
\newcommand{\nbbm}{\ensuremath{\mathbbm{n}}}
\newcommand{\obbm}{\ensuremath{\mathbbm{o}}}
\newcommand{\pbbm}{\ensuremath{\mathbbm{p}}}
\newcommand{\qbbm}{\ensuremath{\mathbbm{q}}}
\newcommand{\rbbm}{\ensuremath{\mathbbm{r}}}
\newcommand{\sbbm}{\ensuremath{\mathbbm{s}}}
\newcommand{\tbbm}{\ensuremath{\mathbbm{t}}}
\newcommand{\ubbm}{\ensuremath{\mathbbm{u}}}
\newcommand{\vbbm}{\ensuremath{\mathbbm{v}}}
\newcommand{\wbbm}{\ensuremath{\mathbbm{w}}}
\newcommand{\xbbm}{\ensuremath{\mathbbm{x}}}
\newcommand{\ybbm}{\ensuremath{\mathbbm{y}}}
\newcommand{\zbbm}{\ensuremath{\mathbbm{z}}}
%%%numbers \mathbbm
\newcommand{\zerobbm}{\ensuremath{\mathbbm{0}}}
\newcommand{\onebbm}{\ensuremath{\mathbbm{1}}}
\newcommand{\twobbm}{\ensuremath{\mathbbm{2}}}
\newcommand{\fourbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\fifebbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\sixbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\sevenbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\eightbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\ninebbm}{\ensuremath{\mathbbm{3}}}


%%%capital \mathbm
\newcommand{\Abm}{\ensuremath{\bm{A}}}
\newcommand{\Bbm}{\ensuremath{\bm{B}}}
\newcommand{\Cbm}{\ensuremath{\bm{C}}}
\newcommand{\Dbm}{\ensuremath{\bm{D}}}
\newcommand{\Ebm}{\ensuremath{\bm{E}}}
\newcommand{\Fbm}{\ensuremath{\bm{F}}}
\newcommand{\Gbm}{\ensuremath{\bm{G}}}
\newcommand{\Hbm}{\ensuremath{\bm{H}}}
\newcommand{\Ibm}{\ensuremath{\bm{I}}}
\newcommand{\Jbm}{\ensuremath{\bm{J}}}
\newcommand{\Kbm}{\ensuremath{\bm{K}}}
\newcommand{\Lbm}{\ensuremath{\bm{L}}}
\newcommand{\Mbm}{\ensuremath{\bm{M}}}
\newcommand{\Nbm}{\ensuremath{\bm{N}}}
\newcommand{\Obm}{\ensuremath{\bm{O}}}
\newcommand{\Pbm}{\ensuremath{\bm{P}}}
\newcommand{\Qbm}{\ensuremath{\bm{Q}}}
\newcommand{\Rbm}{\ensuremath{\bm{R}}}
\newcommand{\Sbm}{\ensuremath{\bm{S}}}
\newcommand{\Tbm}{\ensuremath{\bm{T}}}
\newcommand{\Ubm}{\ensuremath{\bm{U}}}
\newcommand{\Vbm}{\ensuremath{\bm{V}}}
\newcommand{\Wbm}{\ensuremath{\bm{W}}}
\newcommand{\Xbm}{\ensuremath{\bm{X}}}
\newcommand{\Ybm}{\ensuremath{\bm{Y}}}
\newcommand{\Zbm}{\ensuremath{\bm{Z}}}
%%%small \mathbm
\newcommand{\abm}{\ensuremath{\bm{a}}}
\newcommand{\bbm}{\ensuremath{\bm{b}}}
\newcommand{\cbm}{\ensuremath{\bm{c}}}
\newcommand{\dbm}{\ensuremath{\bm{d}}}
\newcommand{\ebm}{\ensuremath{\bm{e}}}
\newcommand{\fbm}{\ensuremath{\bm{f}}}
\newcommand{\gbm}{\ensuremath{\bm{g}}}
\newcommand{\hbm}{\ensuremath{\bm{h}}}
\newcommand{\ibm}{\ensuremath{\bm{i}}}
\newcommand{\jbm}{\ensuremath{\bm{j}}}
\newcommand{\kbm}{\ensuremath{\bm{k}}}
\newcommand{\lbm}{\ensuremath{\bm{l}}}
\newcommand{\mbm}{\ensuremath{\bm{m}}}
\newcommand{\nbm}{\ensuremath{\bm{n}}}
\newcommand{\obm}{\ensuremath{\bm{o}}}
\newcommand{\pbm}{\ensuremath{\bm{p}}}
\newcommand{\qbm}{\ensuremath{\bm{q}}}
\newcommand{\rbm}{\ensuremath{\bm{r}}}
\newcommand{\sbm}{\ensuremath{\bm{s}}}
\newcommand{\tbm}{\ensuremath{\bm{t}}}
\newcommand{\ubm}{\ensuremath{\bm{u}}}
\newcommand{\vbm}{\ensuremath{\bm{v}}}
\newcommand{\wbm}{\ensuremath{\bm{w}}}
\newcommand{\xbm}{\ensuremath{\bm{x}}}
\newcommand{\ybm}{\ensuremath{\bm{y}}}
\newcommand{\zbm}{\ensuremath{\bm{z}}}


%%%diverse mathematical symbols and commands
\newcommand{\defas}{\mathrel{\mathop :}=} % ``defined as''-symbol
\newcommand{\asdef}{=\mathrel{\mathop :}} % ``as defined''-symbol
%\newcommand{\op}[1]{\hat{\mathrm{#1}}}
\newcommand{\opsf}[1]{\hat{\mathsf{#1}}}

%\newcommand{\bra}[1]{\langle #1 |}
%\newcommand{\ket}[1]{| #1 \rangle}

\renewcommand{\d}{\ensuremath{\mathrm{d}}}
%\newcommand{\ee}{\ensuremath{\mathrm{e}}}

\newcommand{\sumint}[1]{\underset{#1}{\sum\hs{-4.6mm}\int\hs{0.8mm}}}
\newcommand{\juu}{{1\hspace{-0.54ex}\mathrm{l}\hspace{-0.30ex}\mathrm{l}}} % big matrix one (three lines)
\newcommand{\hph}[1]{\hphantom{#1\;\,}}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\eps}{\varepsilon}
\newcommand{\const}{\mathrm{const}}

%%%diverse mathematical functions / operators
%\newcommand{\Tr}{\ensuremath{\mathrm{Tr}}}
%\newcommand{\tr}{\ensuremath{\mathrm{tr}}}
\newcommand{\sign}{\ensuremath{\mathrm{sign}}}
\newcommand{\diag}{\ensuremath{\mathrm{diag}}}
\newcommand{\Vol}{\ensuremath{\mathrm{Vol}}}
\newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}

%%%diverse physical energy units
\newcommand{\mueV}{\ensuremath{\mu\mathrm{eV}}}
\newcommand{\meV}{\ensuremath{\mathrm{meV}}}
\newcommand{\keV}{\ensuremath{\mathrm{keV}}}
\newcommand{\MeV}{\ensuremath{\mathrm{MeV}}}
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}}
\newcommand{\TeV}{\ensuremath{\mathrm{TeV}}}
\newcommand{\PeV}{\ensuremath{\mathrm{PeV}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%MISCELLANEOUS
\newcommand{\ub}[3]{\underbrace{#1}_{\phantom{#3}\,#2\,#3}}
\newcommand{\ob}[3]{\overbrace{#1}^{\phantom{#3}\,#2\,#3}}
%\newcommand{\ol}{\overline}
\renewcommand{\u}{\underline}
\newcommand{\os}{\overset}
\newcommand{\us}{\underset}

\newcommand{\cds}{\,\cdot\,}

\newcommand{\eg}{e.g.}
\newcommand{\ie}{i.e.}
\newcommand{\etal}{et al.}
\newcommand{\hc}{{\rm H.c.}}
\newcommand{\rhs}{r.h.s.}
\newcommand{\lhs}{l.h.s.}
\newcommand{\wrt}{w.r.t.}
\newcommand{\cf}{cf.}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}


\setlength{\parskip}\smallskipamount
\linespread{1.05}

\setlength{\footnotesep}{3.5mm}


\settimeformat{ampmtime}

\usepackage{float}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\FK}[1]{\color{orange}{#1\;}\color{black}}
\newcommand{\BC}[1]{\color{red}{#1\;}\color{black}}


\newcommand{\Blue}[1]{\textcolor{DARKBLUE}{\sffamily #1}}
\newcommand{\mathblue}[1]{\textcolor{DARKBLUE}{#1}}
\newcommand{\YT}[1]{\textcolor{DARKBLUE}{\sffamily [YT: #1]}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ga{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\la{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\betap{\tilde\beta}
\def\del{\delta_{\rm PBH}^{\rm local}}
\def\Msun{M_\odot}
\def\LQCD{\Lambda_{\rm QCD}}
\def\tQCD{t_{\rm QCD}}
\def\fPBH{f_{\rm PBH}}
\def\MPBH{M_{\rm PBH}}
\def\Gsph{\Gamma_{\rm sph}}
\def\Teff{T_{\rm eff}}
\def\Tth{T_{\rm th}}
\def\aW{\alpha_{\rm W}}
\def\dCP{\delta_{\rm CP}}
\def\nB{n_{\rm B}}
\def\OR{\Omega_{\rm R}}
\def\OM{\Omega_{\rm M}}
\def\OB{\Omega_{\rm B}}
\def\OPBH{\Omega_{\rm PBH}}
\def\ODM{\Omega_{\rm DM}}
\newcommand{\tcb}{\textcolor{blue}}
\newcommand{\sv}{\langle\sigma v \rangle}

%\def\fPBH{f_{\rm PBH}}

\newcommand{\com}{\Ccal}

\newcommand{\Mpl}{M_\mathrm{Pl}}
\newcommand{\dS}{\mathrm{dS}}
\newcommand{\ns}{n_\mathrm{s}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% ******************************************************
% ********************** END HEADER *************************
% ******************************************************

